Changes to the Facebook Algorithm Decreased News Visibility Between 2021-2024

Platforms, especially Facebook, are primary news sources in the US. In its widely criticized "War on News," Meta algorithmically deprioritized news and political content. We use data from 40 news organizations (5,243,302 Facebook posts, 7,875,372,958 user reactions) and 21 non-news pages (396,468 posts; 1,909,088,308 reactions) between January 1, 2016 and February 13, 2025 to examine how these changes influenced news visibility on the platform. Reactions to news declined by 78% between 2021 and 2024 while reactions to non-news pages increased, indicating targeted suppression of news visibility. Low-quality sources were especially suppressed, yet the 2025 end to "War on News" increased user reactions to news, especially low-quality ones. These changes do not reflect decreased news supply, Facebook user base, or interest in news over this period.

==> parts/extra.tex <==
\section*{Ethics Statement}
Our research leveraged a dataset gathered from publicly available Facebook accounts owned by nationally prominent organizations. Aside from information pertaining to specific news organizations, we present all findings at the aggregate level, focusing on population-wide trends rather than insights into individual private users. To maintain transparency and facilitate reproducibility, we will make the entire dataset, including Facebook Post IDs, and the associated code publicly accessible upon the acceptance of our study.

%Nonetheless, we recognize that our work could potentially be misused, particularly in the context of identifying protected attributes like race or gender. We have taken careful measures to ensure our research is ethically conducted.

\section{Paper Checklist to be included in your paper}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
 \item Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
 \answerYes{Yes}
 \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
 \answerYes{Yes}
 \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
 \answerYes{Yes. Refer Methods}
 \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
 \answerYes{Yes. See limitations}
 \item Did you describe the limitations of your work?
 \answerYes{Yes. Refer limitations}
 \item Did you discuss any potential negative societal impacts of your work?
 \answerYes{Yes. See Ethics Statement}
 \item Did you discuss any potential misuse of your work?
 \answerYes{Yes. See Ethics Statement}
 \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
 \answerYes{Yes. See Ethics Statement}
 \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
 \answerYes{Yes and we ensured that the paper conforms to them.}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
 \item Did you clearly state the assumptions underlying all theoretical results?
 \answerNA{NA}
 \item Have you provided justifications for all theoretical results?
 \answerNA{NA}
 \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
 \answerNA{NA}
 \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
 \answerYes{Yes. Refer Discussion and Limitations.}
 \item Did you address potential biases or limitations in your theoretical framework?
 \answerYes{Yes. See limitations}
 \item Have you related your theoretical results to the existing literature in social science?
 \answerYes{Yes. See Discussion}
 \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
 \answerYes{Yes. See Discussion}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
 \item Did you state the full set of assumptions of all theoretical results?
 \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
 \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
 \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
 \answerYes{Yes}
 \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
 \answerNA{NA}
 \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
 \answerNA{NA}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
 \answerYes{Yes. Models to infer hostile expression required GPU usage and hence, relied on 2xA40 48GB GPUs.}
 \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
 \answerYes{Yes. See Discussions.}
 \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
 \answerYes{Yes. See Limitations.}
 
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
 \item If your work uses existing assets, did you cite the creators?
 \answerYes{Yes. We made sure to cite creators.}
 \item Did you mention the license of the assets?
 \answerNA{NA}
 \item Did you include any new assets in the supplemental material or as a URL?
 \answerYes{Yes. Refer Data and Methods}
 \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
 \answerYes{Yes. Data used was curated from publicly available sources.}
 \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
 \answerYes{Yes. See Ethics Statement}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR?
\answerNA{NA}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset? 
\answerNA{NA}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
 \item Did you include the full text of instructions given to participants and screenshots?
 \answerNA{NA}
 \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
 \answerNA{NA}
 \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
 \answerNA{NA}
 \item Did you discuss how data is stored, shared, and deidentified?
 \answerNA{NA}

\end{enumerate}
\end{enumerate}


==> parts/significance.tex <==
% We challenge the dominant narratives on the prevalence of and engagement with negative news on social media. 
% We use \num{6081134} Facebook posts published during four years by 97 news outlets in six countries to show that
% (1)~negative news is a relatively small fraction (12.3\%); 
% (2)~U.S. news is less negative than news in the other countries (39\% lower odds); 
% (3)~Negative news gets 15\% fewer likes and 14\% fewer comments than non-negative news. 
% (4)~Our simulations further shows that only between 5\% to 25\% of engagement is linked to negative 
% news.
